REALM: Reliable Expertise-Aware Language Model Fine-Tuning from Noisy Annotations

Supervised fine-tuning of large language models relies on human-annotated data, yet annotation pipelines routinely involve multiple crowdworkers of heterogeneous expertise. Standard practice aggregates labels via majority vote or simple averaging, discarding annotator identity and causing the model to absorb the errors of unreliable annotators into its parameters. We propose REALM, which jointly learns the model parameters and a scalar expertise value for each annotator, entirely unsupervised and requiring nothing beyond annotator identity. The key idea is to model each observed label as a mixture between the model's prediction and a uniform random guess, weighted by the annotator's learned expertise. REALM applies to any task with a fixed label set, and extends to multiple tasks via a learned expertise matrix. On four text-classification datasets with \emph{real} crowdsourced annotations, REALM is the best method in all $12$ configurations of the three heterogeneous-annotator datasets, improving on the strongest applicable baseline, including majority vote and Dawid--Skene aggregation, by $+2.9$ points on average. On five question answering benchmarks with simulated noisy labels, it outperforms naive noisy fine-tuning in $152$ of $162$ configurations, by $+5.0$ points on average, with gains that grow with model capacity. The learned expertise additionally recovers annotator reliability without ever observing it. Our code is available at https://github.com/sajjad-ucsb/REALM

==> src/future.tex <==
\section{Future Work}
\paragraph{Efficient and Distributed Fine-Tuning.}
Fine-tuning large language models at scale introduces practical
challenges beyond data quality, including communication overhead,
privacy constraints, and computational efficiency.
In many real-world annotation pipelines, training data is collected
from multiple independent sources or organizations, each with its own
data distribution and annotation practices, mirroring the federated
learning setting where data heterogeneity across clients is a central
challenge.
Recent work has extended parameter-efficient fine-tuning methods to
federated \cite{ghiasvand2025communication} and fully decentralized settings
\cite{ghiasvand2025decentralized}, with explicit mechanisms for handling
non-i.i.d.\ data distributions and convergence guarantees.
The data heterogeneity problem in these settings is conceptually
related to the annotator heterogeneity problem studied in this paper:
in both cases, a model must be trained on data from multiple sources
of varying quality without access to a unified gold standard.
REALM addresses this at the annotation level by learning per-source
reliability weights, and combining expertise-aware objectives with
federated optimization represents a natural direction for future work.

\paragraph{State-Dependent Expertise.}
In REALM, each annotator is assigned a single scalar expertise value
$\beta_i$ that is constant across all prompts.
This is a simplifying assumption: in practice, an annotator may be
highly reliable on certain question types or domains while performing
poorly on others, even within the same dataset.
A natural extension is to model expertise as a function of the input,
$\rho_i(Q) = \sigma(\langle f_\phi(Q), \omega_i \rangle)$, where
$f_\phi(Q)$ is a learned embedding of the prompt and $\omega_i$ is a
per-annotator skill vector.
This formulation allows the model to identify not just \emph{who} is
reliable, but \emph{when} each annotator can be trusted, enabling
finer-grained down-weighting that adapts to the difficulty and domain
of each individual example.
In the multi-task setting, this would remove the requirement that the
task assignment $f^*(Q)$ be observed at training time, as the model
could infer task identity implicitly from the prompt representation.
